Multiple zeta values in deformation quantization

Kontsevich's 1997 formula for the deformation quantization of Poisson brackets is a Feynman expansion involving volume integrals over moduli spaces of marked disks. We develop a systematic theory of integration on these moduli spaces via suitable algebras of polylogarithms, and use it to prove that Kontsevich's integrals can be expressed as integer-linear combinations of multiple zeta values. Our proof gives a concrete algorithm for calculating the integrals, which we have used to produce the first software package for the symbolic calculation of Kontsevich's formula.

==> dq-weights-integration.tex <==
\subsection{The de Rham isomorphism for polylogarithms}

We now turn to the study of polylogarithmic differential forms on $\C{P,Q}$. As was the case for analytic functions, the pullback
\[
\iota^* : \iota^{-1}\sforms{\M{S}} \to \sforms{\C{P,Q}}
\]
on sheaves of differential forms in injective.  In particular, we have the algebra of Arnold forms
\[
\A{\C{P,Q}} := \iota^*\A{\M{S}} \subset \forms{\C{P,Q}}
\]
and the complex of sheaves
\[
\VAr{P,Q} := \iota^*\VAr{S} \cong \Vr{P,Q} \otimes \A{\C{P,Q}} \subset \sforms{\C{P,Q}}
\]
consisting of $\Vr{P,Q}$-linear combinations of Arnold forms. Note that by \autoref{thm:koszul-homotopy} and \autoref{cor:VPQ-acyc}, the complex $\VAr{P,Q}$ is an acyclic resolution of the constant sheaf  $\MZVipi$ on $\C{P,Q}$.   Hence, if we denote by 
\[
\VA{\C{P,Q}} := \sect{\C{P,Q},\VAr{P,Q}} \subset \forms{\C{P,Q}}
\]
the complex of global sections, have the following refinement of the de Rham isomorphism:
\begin{theorem}
The filtered complex $(\VA{\C{P,Q}},\td)$ computes the singular cohomology of $\C{P,Q}$ with coefficients in the filtered ring $\MZVipi\subset \CC$.
\end{theorem}
Similar statements evidently hold for the individual fibres of a projection, where the coefficients $\MZVipi$ are replaced with the corresponding space of germs of polylogarithms on the base.


\subsection{Fibre integration}

Suppose that $P \subset P'$ and $Q \subset Q'$ are inclusions of finite sets, where $Q'$ is totally ordered.  Let 
\begin{align*}
n_P &:= |P'\setminus P| & n_Q &:= |Q'\setminus Q|
\end{align*}
be the difference in the cardinalities.
Then the fibres of the natural projection
\[
	f : \C{P',Q'} \to \C{P,Q}
\]
are manifolds of dimension
\[
d := 2n_P + n_Q.
\]

Suppose that $\omega \in \forms{\C{P',Q'}}$ is a differential form.  Recall that the pushforward of $\omega$ is the differential form $f_*\omega \in \forms[\bullet-d]{\C{P,Q}}$ obtained by integrating $\omega$ over the fibres of $f$.  Note that since the fibres are not compact, the fibre integrals defining the pushforward are not guaranteed to converge, and hence the pushforward may not exist in general.  However, we will only need to deal with the case in which the pushforward $f_*\omega$ converges absolutely.

The main result of the paper is the following:
\begin{theorem}\label{thm:pushforward}
Suppose that $\omega \in \VA[j][k]{\C{P',Q'}}$ is such that the pushforward $f_*\omega$ converges absolutely.  Then
\[
f_*\omega \in \VA[j-2n_P-n_Q][k-n_P]{\C{P,Q}}.
\]
\end{theorem}

Specializing to the case of a projection to a point, we have the following immediate
\begin{corollary}
Suppose that $\omega \in \A[d]{\C{P,Q}}$, where $d = \dim \C{P,Q}$.  Then
\[
\int_{\C{P,Q}} \omega \in \begin{cases}
\MZVipi[|P|-1] & |Q| \le 1 \\
\MZVipi[|P|+|Q|-2] & |Q| \ge 2
\end{cases}
\]
\end{corollary}
\begin{proof}[Proof of corollary]
As long as $|Q| \ge 2$, the moduli space $\C{P,Q}$ projects to $\C{0,2} \cong \{*\}$.  In this case $n_P = |P|$ and $n_Q = |Q|-2$.  On the other hand, if $Q < 2$, then we must have $|P| \ge 1$ and hence there is a projection to $\C{1,0} \cong \{*\}$, for which $n_P = |P|-1$ and $n_Q = |Q|$.  The result follows since $\omega \in \VA[2|P|+|Q|-2][2|P|+|Q|-2]{\C{P,Q}}$ and $\VA{\C{1,0}} = \VA{\C{0,2}} = \MZVipi$.
\end{proof}

We now turn to the proof of \autoref{thm:pushforward}.  The strategy is as follows. First, recall that if $\alpha \in \forms{\C{P,Q}}$ is a form on the base, then Fubini's theorem gives the projection formula
\[
f_*(\alpha \wedge \omega) = \alpha \wedge f_*\omega
\]
whenever $f_*\omega$ converges absolutely.  Hence by induction, the theorem reduces to the case in which $f$ is one of the elementary projections in which a single boundary or interior marked point is forgotten.  Furthermore, thanks to the Arnold relations,  $\VA[\ge d]{P,Q}$ is generated by $\VA[d]{P,Q}$ as an $\A{\C{P,Q}}$-module.   Hence it is enough to consider the pushforward of forms whose degree is equal to the dimension of the fibres.  We treat these cases by constructing a primitive for $\omega$ along the fibres, and applying Stokes theorem.



\subsubsection{Pushforward along interval fibres}

Consider a projection $f_q : \C{P',Q'} \to \C{P,Q}$ that forgets a single marked point $q \in Q$ as in \autoref{sec:acyc-bdry}.  We have the following:
\begin{proposition}
Suppose that $\omega \in \VA[1][k]{\C{P',Q'}}$ is such that $f_*\omega$ converges absolutely.  Then $f_*\omega \in \VA[0][k]{\C{P,Q}}$.
\end{proposition}

\begin{proof}
Recall from \autoref{sec:acyc-bdry} that the fibres of $f_q$ are given by the open intervals in the universal curve $\uXo{S}$, in which the marked point $q$ moves between its neighbouring boundary marked points $q_- < q < q_+$.  Let $\alpha \in \V{\C{P',Q'}}$ be a fibrewise primitive for $\omega$ as in \autoref{thm:fibre-prim}.  Then by the fundamental theorem of calculus, the pushforward is given by
\begin{align}
f_*\omega = \int_{q_- < q < q_+} \omega =  (\lim_{q \to q_+} -\lim_{q \to q_-}) \alpha. \label{eqn:int-push-limits}
\end{align}
The limits exist since we assume that $f_*\omega$ is absolutely integrable, and by  \autoref{thm:rlims} they give polylogarithms on the base of weight at most $k$.
\end{proof}

The pushforward can be calculated algorithmically as follows.  Note that the differential forms $\dlog{s}$ for $s \in S$ give a basis for the relative differentials of the projection.  Thus by using $q_-$ as a base point for hyperlogarithms in the fibres, we obtain a unique expansion
\[
\omega = \sum_{s \in S} L_{u_s} \dlog{s} \mod f^*\forms[1]{\C{P,Q}}
\]
where $L_{u_s} \in \V[k-1]{\C{P,Q}}$ denotes the hyperlogarithm associated to an element $u_s \in \V{\C{P,Q}}\abrac{S}$.  We may therefore construct a natural primitive for $\omega$ by adding the symbol $s$ to the end of each element $u_s$, giving a function
\[
\alpha := \sum_s L_{u_ss} \in \V[k]{\C{P',Q}}
\]
such that $\td \alpha = \omega$.  The limits in \eqref{eqn:int-push-limits} can then be computed following the recipe in \autoref{???}

\subsubsection{Pushforward along disk fibres}

\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{Graphs/contour}
	\caption{The integration domain.}%
	\label{fig:contour}%
\end{figure}
We now consider a projection
\[
f : \C{P',Q'} \to \C{P,Q}
\]
in which a single interior marked point is forgotten as in \autoref{sec:acyc-int}.  The fibres can be canonically compactified by adding in the boundary of the disk and filling in the marked points.  In this way we obtain the universal marked disk over $\C{P,Q}$.  For the purposes of integration, it is convenient to perform a real oriented blow up of the universal marked disk at its marked points.  This results in a fibration by surfaces with boundary and corners.  whose codimension-one boundary faces come in three types:
\begin{itemize}
\item Circles $\eta_p$ for $p \in P$, which blow down to the interior marked points
\item Half-circles $\sigma_q$ for $q \in Q \cup \{\infty\}$, which blow down to the boundary marked points
\item Segments $\gamma_q$  for $q \in Q \cup \{\infty\}$, which blow down to the intervals connecting a boundary marked point $q \in Q\cup \{\infty\}$ with its successor in the cyclic order
\end{itemize}
The inclusion $\C{P',Q} \to \M{S'}$ extends to a map of this space to $\bM{S'}$.  The Each of the intervals $\gamma_q$ maps to an interval in the universal curve over 


The boundary circles $\eta_p$ are contracted to points, while the 

so that the total boundary cycle is given by
\[
\partial 
\]
The case $|P| = |Q| = 3$ is illustrated in \autoref{fig:blowup-disk}.

\begin{figure}
\begin{center}
\begin{tikzpicture}
\def\Rad{4}
\def\rad{0.75}
% Node positions
\node (q1) at (-130:\Rad) {};
\node (q2) at (-70:\Rad) {};
\node (q3) at (-20:\Rad) {};
\node (qinf) at (90:\Rad) {};

% Fill the interior
\draw[fill=lightgrey] (0,0) circle (\Rad);

% Draw real line boundary arcs
\placeoutseg{q1}{-130}{-70}{$\gamma_{q_1}$}
\placeoutseg{q2}{-70}{-20}{$\gamma_{q_2}$}
\placeoutseg{q3}{-20}{90}{$\gamma_{q_3}$}
\placeoutseg{qinf}{90}{230}{$\gamma_\infty$}

% Cut out interior circles
\placeinterior{1}{30:0.5*\Rad}
\placeinterior{2}{160:0.6*\Rad}
\placeinterior{3}{-50:0.3*\Rad}

% Cut out boundary half-circles
\placeoutpt{q1}{$q_1$}
\placeoutpt{q2}{$q_2$}
\placeoutpt{q3}{$q_3$}
\placeoutpt{qinf}{$\infty$}
\clip (0,0) circle (\Rad);
\placeoutarc{q1}{-130}{$\sigma_{q_1}$}
\placeoutarc{q2}{-70}{$\sigma_{q_2}$}
\placeoutarc{q3}{-20}{$\sigma_{q_3}$}
\placeoutarc{qinf}{90}{$\sigma_\infty$}
\end{tikzpicture}
\end{center}
\caption{The surface with boundary and corners obtained by blowing up a marked disk}
\label{fig:blowup-disk}
\end{figure}

filling in the punctures and performing a real-oriented blowup 

 which can be compactified by filling in the punctures and performing a real-or

In the compactification $\C{P',Q}$ the fibres of 

\begin{proposition}
Suppose that $\omega \in \VA[2][k]{\C{P',Q'}}$ is such that $f_*\omega$ converges absolutely.  Then $f_*\omega \in \VA[0][k-1]{\C{P,Q}}$
\end{proposition}

We break the proof into a sequence of lemmas, which together give an algorithm for calculating the pushforward.  Note that it is sufficient to consider the pushforward of $\omega$ over a contractible open set $\U \subset \C{P,Q}$.

To begin, note that using the complex conjugate coordiantes $(z,\zb)$ on the fibres, there is a natural Dolbeault decomposition of one-forms along the fibres into forms of type $(0,1)$ and $(1,0)$.
\begin{lemma}
The form $\omega$ admits a primitive $\alpha \in \VAr[1][k]{P',Q'}(f^{-1}(\U))$ that restricts to a single-valued $(1,0)$-form on each fibre.
\end{lemma}

\begin{proof}
The obstruction is in $H^2$ of the fibres, which vanishes.  A primitive can be constructed algorithmically as follows.  Consider the double complex...
\end{proof}

Since $f_*\omega$ converges absolutely, we have by Stokes theorem that the integral over any fibre is given by
\[
f_*\omega = \lim_{\epsilon \to 0} \int_{\gamma_\epsilon} \alpha
\]
where $\gamma_\epsilon$ is the one-cycle shown in \autoref{fig:contour}.  It is composed of three types of elementary pieces:
\begin{itemize}
\item circles of radius $\epsilon$ around each interior marked point $p \in P$
\item half-circles of radius $\epsilon$ around each boundary marked point $q \in Q \cup \sset{\infty}$
\item intervals between neighbouring pairs of marked points on the boundary
\end{itemize}
We now treat each of these cases in turn.

\paragraph{Interior circles:}  Note that any $(1,0)$-form in the Arnold algebra restricts to a linear combination of the forms $\frac{\td z}{(2\ipi)(z-s)}$ on the fibres, where $s \in S$.  Hence $\alpha \in \Vr[k-1]{P,Q}\otimes \A[1]{\C{p,Q}}$ can be written uniquely in the form
\[
\alpha = \sum_{s \in S}  \frac{\alpha_s(z,\zb)\td z}{(2\ipi)(z-s)}  \mod f^*\forms[1]{\C{P,Q}}
\]
where the coefficients $\alpha_s \in \Vr[k-1]{P',Q'}$ are polylogarithms.  We may then define a residue for $\alpha$ at an interior marked point $p\in P$ by extracting the (regularized) coefficient of $\tfrac{\td z}{z-p}$:
\[
\Res_{p}\alpha := \Rlim_{z \to p}\Rlim_{\zb \to \pb} \frac{\alpha_p(z,\zb)}{2\ipi} \in \frac{1}{2\ipi}\Vr[k-1]{P,Q}
\]
Note that if $\alpha$ has weight $k$, then $2\ipi \Res_p\alpha \in \Vr[k-1]{P,Q}$ is a polylogarithm on the base $\C{P,Q}$ of weight $k-1$.

We have the following analogue of the residue theorem, which we learned from the paper \cite{Schnetz2014} of Schnetz:
\begin{lemma}
Suppose that $\alpha \in \VAr[1]{P',Q'}$ is a single-valued polylogarithmic that has type $(1,0)$ in the fibre coordinates $(z,\zb)$.  Let $\delta(\epsilon)$ be a positively oriented circle of radius $\epsilon$ centred at $p$ in some fibre.  Then we have
\[
\Rlim_{\epsilon \to 0} \int_{\delta(\epsilon)}  \alpha = 2 \ipi \Res_p\alpha 
\]
\end{lemma}

\begin{proof}[Sketch of proof]
Using shuffle regularization, one can expand $\alpha = g(z) \tfrac{\td z}{z-p}$ where $g$ is a polynomial in $\log(z-p)$ and $\log(\zb - \pb)$, with coefficients that are analytic at $p$.  Since $\alpha$ is single-valued, one can check that this expansion must in fact reduce to a polynomial in the single-valued logarithm $\log |z-p| = \log \epsilon$.  One then uses this expansion to compute the asymptotics of the integral as $\epsilon \to 0$, giving the result.  The details of the analysis are essentially the same as in \cite[Section 2.8]{Schnetz2014}, so we shall omit them.
\end{proof}
%
%\begin{proof}
%Since $\alpha \in \Vr[k-1]{P',Q'}\otimes \A[1]{\C{P',Q'}}$ is a $(1,0)$-form, it is a $\Vr{P',Q'}$-linear combination of the differential forms $\invtate\frac{\td z}{z-s}$ for $s \in S$.  Hence we may write
%\[
%\alpha = L_j(z,\zb) g_j(z,zb)  \frac{dz}{(2\ipi)(z-p)} 
%\]
%where $g$ is holomorphic at $p$ and $L \in \Vr[k-1]{P',Q'}$ is single-valued on the punctured disk.  Writing $L$ in the fibration basis as in \eqref{eq:disk-fibration-basis} and applying shuffle regularization to the hyperlogarithm factors at the possible singularities $z=p$ and $\zb=\pb$, we see that $L$ admits an expansion of the form
%\[
%L = \sum_{j=0}^N\sum_{k=0}^M \frac{1}{j!k!}\rbrac{\frac{\log(z-p)}{2\ipi}}^j \rbrac{\frac{\log(\zb-\pb)}{2\ipi}}^k h_{jk}(z,\zb)
%\]
%where $h_{jk}$ are real analytic at $p_0$.  The fact that $L$ is single-valued in a neighbourhood of $p$ implies, by a straightforward inductive argument, that  $h_{j,k} = 0$ whenever $j \ne k$, so that $L$ reduces to a polynomial in $\log(z-p)\log(\zb-\pb) = 2\log r$ where $r = |z-p|$ is the radial distance from $p$:
%\[
%L = \sum_{j=0}^N \tfrac{2^j}{j!}  h_j(z,\zb) \log^j r
%\]
%Note than since the functions $h_j$ and $g$ are analytic at $p$, and the circumfrence of $\delta(\epsilon)$ vanishes linearly with $\epsilon$, the standard residue calculation gives
%\[
%\lim_{\epsilon \to 0}\int_{\delta(\epsilon)} h_j(z,\zb)g(z) \frac{\td z}{(2\ipi)(z-p)} = h_j(p,\pb)g(p)
%\]
%Since $r = \epsilon$ is constant on the path $\delta(\epsilon)$, we therefore have
%\begin{align*}
%\lim_{\epsilon \to 0} \int_{\delta(\epsilon)} \alpha &= \lim_{\epsilon \to 0} \frac{(2 \log \epsilon)^j}{j!} \int h_j(z,\zb)g(z) \frac{\td z}{z-p} \\
%&= \lim_{\epsilon \to 0} \frac{(2 \log \epsilon)^j}{j!} h_j(p,\pb)g(p)
%\end{align*}
%This limit is divergent unless $h_j(p,\pb) =0$ for $j > 0$, but we know a priori that the limit exists.  We conclude that 
%\end{proof}

\paragraph{Boundary cycle:}

The other boundary component consists of a collection of intervals.


\begin{lemma}
half-residue
\end{lemma}

By construction $\alpha$ has an expansion around $p_0$ consisting of terms of the form
\[
f^*a \log^j|z-p_0|(z-p_0)^j(\zb-\pb_0)^k \frac{\td z}{(2 \ipi)z-p_0}
\]

 the terms of the form 
where 
By shuffle regularization, the polylogarithmic coefficients of $\alpha$ admit an expansion in powers of $\log(z-p)$ and $\log(\zb - \pb)$ near $p$.  Meanwhile, the one-form part has at worst a simple pole at $p$.  Hence $\alpha$ admits an expansion of the form
\[
\alpha = \sum_{lm} \frac{a_{mn}}{m!n!}\rbrac{\frac{\log(z-p)}{2\ipi}}^m\rbrac{\frac{\log(\zb-\pb)}{2\ipi}}^n  \frac{\td z}{(2\ipi)(z-p)}
\]
where
\[
a_{mn} \in f^*\V[k-1]{\C{P,Q}} \mod (z-p)
\]

By shuffle regularization, $\alpha$ has an expansion
The only one-forms in $\A{\C{P',Q}}$ that 

 so that we may decompose the fibrewise de Rham differential as 
\[
\td = \del + \delb
\]

 We may write
\[
\omega = \sum_{s \in S} \sum_{\st \in S \cup p} L_{s,\st} \frac{\td z }{z-s} \wedge \frac{\td \zb}{\zb -\tilde s} \mod f^*\forms[1]{\C{P,Q}}
\]
where $L_{s,\st}$ is the iterated hyperlogarithm associated with an element
\[
u_{s,\st} \in \V{\C{P,Q}}\abrac{S|P}\abrac{S,p}
\]
We may construct a primitive of $\omega$ with respect to t

 Given a volume form $\omega \in \VA[N]{\C{P',Q}}$ of degree $N=\dim \C{P',Q}$, we decompose it as the product $\omega \in \VA[2]{p} \tp_{\MZVipi} \VA[N-2]{\C{P,Q}}$ \erik{Notation problem: I need a symbol for sv base forms, with Arnol'd forms, that are not necessarily integrable} of forms on the base and two-forms in the fibre, where
\begin{equation*}
	\VA{p} \defas \A{\C{P'/P,Q}} \tp \V{\C{P'/P,Q}}_{\MZVipi}.
\end{equation*}
By Fubini's theorem, we may fix a point $y \in \C{P,Q}$ in the base and integrate over the fibre $F=p^{-1}(y)$. By \autoref{cor:sv-primitives} we can find a primitive $\alpha$ of $\omega|_{F}$ of degree $(0,1)$ in the fibre. That is, picking a representative $y=[(\set{z_i}{i\in P}, \set{p_j}{j\in Q})]$ of $y$, $\alpha \in \A[1]{\set{\td \log (\bar{z}-\sigma)}{\sigma \in \Sigma}}$ where $\Sigma = \set{z_i}{i \in P} \subset \HH$.\erik{How to fix scale of tangential base points?}
\erik{Could we abbreviate the relatives with $\Arel[1]{p}_1$?}

We now apply Stokes theorem to an open $U$ of the kind illustrated by the shaded region in figure~\ref{fig:contour}. Concretely, we set
\begin{equation*}
	U = \set{z \in \HH}{\snorm{z-\sigma} \geq r_{\sigma}\ \text{for all}\ \sigma \in \overline{\Sigma}}
	\cap \sset{\snorm{z}<r_{\infty}}
	\cap \sset{\Im(z) > r_{\RR}}
\end{equation*}
where $\overline{\Sigma} \defas \Sigma \sqcup \set{p_j}{j \in Q}$. We know that
\begin{equation*}
	p_*(\omega) 
	= \lim_{r\rightarrow 0} \int_{U(r)} \omega
	= \lim_{r\rightarrow 0} \int_{\partial U(r)} \alpha
\end{equation*}
The procedure is as follows:
\begin{itemize}
	\item Construct a fibrewise single-valued primitive of $\omega$.  The existence basically follows from Francis' constructions \cite{Brown2004,Brown2004a} on $\PP[1]$ but there is a slight difference because we are working on the upper half-plane $\HH\subset \PP[1]$.  In particular, there is an extra form $\tfrac{\td (z-\zb)}{z-\zb}$ whose iterated integrals can appear.  The explicit algorithm is
\begin{itemize}

\item Construct a primitive $\alpha_j$ of each $\omega_j$, so that $\alpha_j$ has type $(0,1)$ in the Dolbeault decomposition along the fibres.  This corresponds to taking a primitive in $\VA{\tM{0,N}}$ along the fibres of $\M{0,N} \to \M{0,N-1}$ and is easily done in the tensor algebra in the usual way.
\item Cancel the monodromy of the primitive $\sum \alpha_j \wedge p^*\omega'_j$ through the addition of antiholomorphic $(0,1)$-forms.  This is done iteratively, reducing the weight of the monodromy at each step.
\end{itemize}
\item Apply a regularized Stokes theorem in the style of Schnetz.  The fibres are punctured disks, and at each puncture the argument is basically the same as Schnetz' argument on $\PP[1]$.  But the boundary of the disk gives an additional contribution.  It is clear that these contributions lie in $\VA{\C{n-1,m}}$, but an extra argument is needed to show that this contribution has an overall factor of $\pi \iu$. 
	We use a contour deformation argument to see this.
\end{itemize}




\subsubsection{Residues}
The only singular forms at $z=p$ are $\td \log (z-p)$ and $\td \log(\bar{z}-\bar{p})$. It follows directly from the theory of hyperlogarithms that any function $f \in \V{X}$ admits an expansion
\begin{equation*}
	f = \sum_{i,j=0}^N \frac{\log^i(z-p)}{i!} \frac{\log^j(\bar{z}-\bar{p})}{j!}f_{i,j}(z)
\end{equation*}
where $N$ is the tensor degree and $f_{i,j}(z)$ are uniquely determined functions that are real analytic at $z=p$ (they also depend on the base, which we suppress in the notation). In fact, single-valuedness of $f$ around $z=p$ implies that the holomorphic and antiholomorphic logarithms have to combine into
\begin{equation*}
	f=\sum_{k=0}^N \frac{\log^k (z-p)(\bar{z}-\bar{p})}{k!} f_k(z)
\end{equation*}
where $f_k = f_{i,k-i}$ for any $i \leq k$. Since this diverges for small $r \defas \snorm{z-p}$ only like a power of $\ln r$, but the the measure of the integration cycle $\gamma_r(t) = p+r e^{-2\ipi t}$ is proportional to $r$, it follows that $\lim_{r\rightarrow 0} \oint_{\gamma_r} \td \log(\bar{z}-\sigma) \cdot f(z) = 0$ for any $\sigma \neq \bar{p}$.
For $\sigma=\bar{z}$, we get
\begin{equation*}
	\oint_{\gamma_r} \td \log (\bar{z}-\bar{p}) f(z)
	\sim \sum_{k=0}^N \frac{\ln^k r^2}{k!} (2\ipi) f_k(p),
\end{equation*}
where $\sim$ denotes that both sides differ by a function that vanishes at $r=0$.
In particular, we see that the convergence of this integral in the limit $r \rightarrow 0$ requires that $f_k(p)=0$ for all $k>0$. The limit itself is then just given by $2\ipi\cdot f_0(p) \in \VA{\C{P,Q}}(1)$.\erik{It is not clear that this residue itself is integrable over the base! We know that only for the full fibre integral!}
\erik[inline]{Add example}



\subsubsection{Half-residue}
\begin{figure}
	\centering\includegraphics[scale=0.8]{Graphs/wedge}%
	\caption{A wedge! Look how beautiful!}%
	\label{fig:wedge}%
\end{figure}
The geometry is more complicated for a collision of $z$ with a boundary point $q\in Q$, because there three boundary divisors meet: $z=q$, $\bar{z}=q$ and $z=\bar{z}$.
The coordinate $u=\crossrat{z}{\bar{z}}{q}{\infty}=\frac{z-q}{\bar{z}-q}$ resolves these into $u=0$, $u=\infty$ and $u=1$, respectively. Restricted to $\C{P',Q}$, $u$ takes values in $S^1\setminus\sset{1}$, and endpoints of the inverval $\bC{1,1}$ are mapped to the tangential base points $\pm \vec{\iu}_1$.


Given a word in $\T{\Arel[1]{\C{n,m}, p_{10}}_0}$, we can use shuffle-regularization to decompose it into $V \defas \T{\sset{\dlog{0},\dlog{\bar{z}}}} \tp \tilde{T}$, where $\tilde{T}$ is the subalgebra of words not ending in any of $\dlog{0}$ or $\dlog{\bar{z}}$.
\begin{lemma}
	With exception of the empty word, every hyperlogarithm $\int_0^z w$ for a word $w \in \tilde{T}$ vanishes at least like $\mathcal{O}(r)$ for $r\defas \snorm{z} \rightarrow 0$ (keeping $z/\bar{z}$ fixed).
	\label{}
\end{lemma}
For the limit onto $z=0$, we can therefore drop all words that are not completely in $V$. The words in $V$ give products of powers of $\log z$ times iterated integrals $\int_0^z w$ for $w$ not ending in $\dlog{0}$. The latter are scale-invariant, so they equal $\int_0^{z/\bar{z}} w'$ where $w'$ is the word obtained from $w$ by substition of $\dlog{\bar{z}}$ with $\dlog{1}$. Note that we can replace $\log z$ by $\log z/\bar{z} + \log \bar{z}$. Any iterated integral $\int_0^{\bar{z}} w$ with $w$ containing a non-zero letter, also vanishes like $\asyO{\bar{z}}$ as $z\rightarrow 0$. Hence we can project those down to $\log(\bar{z})$-powers, up to vanishing terms.
\begin{corollary}
	An iterated integral $F$ of the kind we consider, admits at $z\rightarrow 0$ an expansion of the form
	\begin{equation}
		F(z) = \sum_{k=0}^N \log^k \bar{z} \cdot \sum_{j} f_{k,j}(u) \cdot F_{k,j}(u,y)
		+ \asyO{\snorm{z}}
		\label{}
	\end{equation}
	where $F_{k,j}$ are functions on the base $y = p(x) \in \C{P,Q}$ (i.e. independent of $z$).
\end{corollary}
So, we can define a regularized restriction onto the boundary divisor 
\begin{equation}
	\bC{1,1} \times \bC{n-1,m}
	\hookrightarrow \partial \bC{n,m}
\end{equation}
by projecting to the convergent terms $k=0$. Any of the other terms would contribute an infinity to the integral of $F/z$ around the half-residue (due to a $\log r$-divergence, if we integrate over a little sector (fixed start- and stop angles)). So, for a case where the integral over the boundary is convergent, the regularized restriction is the actual limit of the function! Therefore, it gives the correct integral!

\begin{lemma}
	If $\omega \in \Omega^2(X)$ for a finite set $\Sigma \subset \HH$ is absolutely integrable over $X=\HH \setminus \Sigma$ and $\omega=\td \alpha$ for a one-form $\alpha\in\Omega^1(X)$ in our space of functions, then the part that has $\td \log \bar{z}$ as rational prefactor admits becomes a polynomial in $\log \bar{z}$ in the limit $z\rightarrow 0$.
	\label{}
\end{lemma}
\begin{proof}
	Consider the finiteness of the integral of $\omega$ over the wedge in figure~\ref{fig:wedge}. We keep the angles and the outer radius fixed, and consider the dependence on the inner radius $r$ when $r\rightarrow 0$. By $\td \alpha=\omega$, this is equal to the integral of $\alpha$ along the boundary of the wedge. Since the contribution from the outer arc is independent of $r$, we only need to look at $A$, $B$ and $C$. Let $\alpha' = \sum_{k=0}^N \td \log \bar{z} \cdot \log^k\bar{z}/k! \cdot f_k(u)$ where $u=z/\bar{z}$ and $f_k$ are polylogarithms of the angle at zero (measured by $z/\bar{z}$). Since these are independent of the radius $\snorm{z}$, the integrals over $A$ and $C$ are simply, via $\log\bar{z} = \log \snorm{z} - 1/2 \log (z/\bar{z})$,
	\begin{align*}
		\int_A \alpha' + \int_C \alpha'
		&= \sum_{k=0}^N \left[f_k(e^{2\iu\phi}) \left( 
			\frac{(\log r - \iu \phi)^{k+1}}{(k+1)!}
			-\frac{(\log R - \iu \phi)^{k+1}}{(k+1)!}
		\right)\right]_{\phi=\alpha}^{\phi=\beta}
		\\
		&= \left( f_N(e^{2\iu\beta}) - f_N(e^{2\iu\alpha}) \right) \frac{\ln^{N+1}r}{(N+1)!}
		+ \asyO{\ln^N r}
		.
	\end{align*}
	The integral over $B$, in contrast, diverges at worst like $\ln^N r$:
	\begin{equation*}
		\int_B \alpha'
		= \int_B \left( -\frac{1}{2} \td \log \frac{z}{\bar{z}} \right)
		\sum_{0 \leq i \leq k\leq N} \frac{\log^i r}{i!} f_k\left( \frac{z}{\bar{z}} \right) \frac{(-1/2) \log^{k-i} (z/\bar{z})}{(k-i)!}
		\in \asyO{\ln^N r}
	\end{equation*}
	The convergence of $\int_{A+B+C} \alpha'$ in the limit $r\rightarrow 0$ therefore requires that $f_N$ is a constant. Since $\oint \td \log \bar{z} \cdot \log^N\bar{z}/N! = 0$ is itself convergent, an induction shows that thus all $f_k$ (for all $0\leq k \leq N$) must be constant.
\end{proof}
In consequence, any single-valued primitive $\alpha$ of an absolutely integrable 2-form $\omega$, behaves near a terrestrial point like a polynomial in $\log\bar{z}$, so the half-residues contribute a linear combination of products of
\begin{equation}
	\int_{-r}^r \td \log \bar{z} \cdot \frac{\log^k \bar{z}}{k!}
	= - \frac{(-\ipi)^{k+1}}{(k+1)!}
	\label{eq:half-res}%
\end{equation}
times functions on the base.


\subsubsection{Restriction to the real line}
\begin{equation}
	\bC{1,0} \times \bC{n-1,m+1}
	\hookrightarrow \partial \bC{n,m}
	\label{}
\end{equation}
Note that, in this situation, after taking the limit to the real line, we are actually in the situation of the projection forgetting a boundary point! Indeed, the integration of the restriction is exactly what we described above for $\C{n,m+1} \rightarrow \C{n,m}$!

\subsubsection{Factor of $2\ipi$}
Let $\alpha^{\hol}$ denote the restriction of $\alpha$ to the left of $0$ and consider its analytic continuation (through $\HH$) around $0$. The only contribution to $\lim_{r\rightarrow 0} \int_{-r}^r \alpha^{\hol}$ comes from the terms with the form $\td \log z$. But near $z=0$, we know from \eqref{eq:half-res} that these are
\begin{equation}
	\alpha^{\hol}
	= \left[ \td \log \bar{z} \cdot \frac{\log^k\bar{z}}{k!} \right]_{z=\bar{z}<0}
	= \td \log z \cdot \frac{(\log z - 2\ipi)^k}{k!}
	\label{}
\end{equation}
modulo terms that do not contribute to the integral in question. But this integrates to
\begin{equation}
	\int_{-r}^r \alpha^{\hol}
	= \left[ \frac{(\log z-2\ipi)^{k+1}}{(k+1)!} \right]_{z=1}^{z=-1}
	= \frac{(-2\ipi)^{k+1}}{(k+1)!} - \frac{(-\ipi)^{k+1}}{(k+1)!}.
	\label{}
\end{equation}
The second term coincides with the half-residue contribution of $\alpha$ itself, and the first term is in $2\ipi\cdot \MZVipi$. So, up to corrections in $\MZVipi(1)$ (or rather $\MZVipi(1) \times \text{base functions}$), we can replace $\alpha$ by $\alpha^{\hol}$ in the half-residue integrals.

Furthermore, we note that the values of $\alpha^{\hol}$ on different connected components of the boundary are connected, through analytic continuation, again by corrections in $\MZVipi(1)$. This follows from the expansion \erik{ref} above, because
\begin{itemize}
	\item The functions $F_{k,w}$ restrict on both sides of $0$ to the same function
	\item $\log\bar{z}|_{z=\bar{z}<0} = \log z - 2\ipi$ extends to the right of $0$ to $\log z - 2\ipi$, which differs from $\log\bar{z}|_{z=\bar{z}>0} = \log z$ by $-2\ipi$
	\item The finiteness of the restriction to the real line $z=\bar{z}$ imply that the polylogs $f_k(z/\bar{z})$ must be finite at $z/\bar{z}\rightarrow 1 \pm \iu\varepsilon$. But this implies that $f_k(1+\iu\varepsilon)-f_k(1-\iu\varepsilon)$ is a monodromy of a polylog on $\M{4}$, and therefore in $\MZVipi(1)$.
\end{itemize}

In consequence, we see that $\int_{C} \alpha \equiv \int_C \alpha^{\hol} \mod \MZVipi(1)$, where $C$ is the component of the boundary $\partial X$ with the real-line intervals. Of course, $\alpha^{\hol}$ is not single-valued along $C$, but the monodromies lie in $\MZVipi(1)$, so this statements make sense for any choice of branch. Now, crucially, $C$ is closed, so $\int_C \alpha^{\hol} = \Mon{C} \eta^{\hol}$ is the monodromy of the holomorphic primitive $\eta^{\hol}$ of $\alpha^{\hol}= \td \eta^{\hol}$. This proves that we get the sought-after factor of $(2\ipi)$.






